Uni-MoE: Scaling Unified Multimodal LLMs with Mixture of Experts

Recent advancements in Multimodal Large Language Models (MLLMs) underscore the significance of scalable models and data to boost performance, yet this often incurs substantial computational costs. Although the Mixture of Experts (MoE) architecture has been employed to efficiently scale large language and image-text models, these efforts typically involve fewer experts and limited modalities. To address this, our work presents the pioneering attempt to develop a unified MLLM with the MoE architecture, named Uni-MoE that can handle a wide array of modalities. Specifically, it features modality-specific encoders with connectors for a unified multimodal representation. We also implement a sparse MoE architecture within the LLMs to enable efficient training and inference through modality-level data parallelism and expert-level model parallelism. To enhance the multi-expert collaboration and generalization, we present a progressive training strategy: 1) Cross-modality alignment using various connectors with different cross-modality data, 2) Training modality-specific experts with cross-modality instruction data to activate experts' preferences, and 3) Tuning the Uni-MoE framework utilizing Low-Rank Adaptation (LoRA) on mixed multimodal instruction data. We evaluate the instruction-tuned Uni-MoE on a comprehensive set of multimodal datasets. The extensive experimental results demonstrate Uni-MoE's principal advantage of significantly reducing performance bias in handling mixed multimodal datasets, alongside improved multi-expert collaboration and generalization. Our findings highlight the substantial potential of MoE frameworks in advancing MLLMs and the code is available at https://github.com/HITsz-TMG/UMOE-Scaling-Unified-Multimodal-LLMs.

==> additional_tables.tex <==
\begin{table*}[t]
\renewcommand\arraystretch{1.15}
\centering
\caption{\label{more-experts-und}
\textbf{Ablation Study of Uni-MoE performances with more image-text training data and experts}. For models with \textit{X}B, \textit{X} refers to the size of the language model.  For our models with \textit{Y}E, \textit{Y} refers to the number of experts.  
Names are abbreviated due to space limits. I: Image; T: Text; A: Audio; S: Speech; V: Video; AOK: A-OKVQA \cite{aokvqa}; OK: OK-VQA~\cite{okvqa}; MMB: MMBench~\cite{mmbench}; POPE~\cite{li-etal-2023-evaluating}; VQA$^T$: TextVQA~\cite{singh2019towards}; SEED:SEED-Bench~\cite{seedBENCH}; MMVet~\cite{yu2023mm}.
``EHSL'' refers to the English High School Listening Test we collected, containing long/short speech types.
$^\ddagger$ indicates that this model employs enormous or unknown data during training.
Uni-MoE still achieves better comprehensive performances, demonstrating the mixed training data management capacities of MoE.}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|cccccccc|ccc}
\hline
\textbf{Method} & \textbf{AOK} & \textbf{OK} & \textbf{VQAv2} & \textbf{MMB} & \textbf{POPE} &\textbf{VQA$^T$} & \textbf{SEED} & \textbf{MMVet} & \textbf{RACE-Audio} & \textbf{EHSL} & \textbf{ActivityNet-QA} \\
\hline
\textit{Any-Modality Understanding} & & & & & & & & &\\
Macaw-LLM~\cite{lyu2023macaw}  & 1.90\% & 5.70\% & 20.73\% & 3.84\% & - & - & - & - & 4.04\%/3.00\% & 0.67\%/2.00\% &  -\\
X-InstructBLIP~\cite{panagopoulou2023x} & 21.52\% & 30.61\% & 37.77\% & 8.96\% & - & - & - & - & 16.33\%/18.88\% & 0.67\%/2.00\% &-\\
\hline
\textit{Dense Model} & & & & & & & & & \\
AnyMAL-70B (I,T,A,V)~\cite{moon2023anymal} & -&42.6\% &64.2\% & -& -& 32.9\% & -&-&-&-&-\\
IDEFICS-80B (I,T)~\cite{laurenccon2024obelics} & - & -& 60.0\% & 54.5\% & - & 30.9\% & -& - & - & - &- \\
LLaVA-1.5-7B (I,T)~\cite{liu2023improved} & 70.92\% & 55.09\% & 75.9\% & 72.7\% & 85.9\% & 58.2\% & -& 30.5\% & -& - & -  \\
LLaVA-1.5-13B (I,T)~\cite{liu2023improved} & 73.54\% & 61.93\% & 78.9\% & 73.4\% & 85.9\% & 60.2\% & - & 35.4\% & -& - & - \\
BLIP-2(FlanT5-xxl)-11B (I,T)~\cite{li2023blip2} & 39.06\% & 53.7\% & 65.0\% & - & 85.3\% & 42.8\% & -&-&-&-&-\\
InstructBLIP(Vicuna)-13B (I,T)~\cite{dai2024instructblip} & 58.30\% & 41.02\% & - & - & 50.7\% &- &25.6\% & - & -& - & -\\
Shikra-13B (I,T)~\cite{chen2023shikra} &- & -& 77.4\% & 58.8\% & - & -&-& - & -& - & -\\
LLaMA-VID-13B (I,T,V)~\cite{li2023llamavid} & -& -& 80.0\%& 66.6\% & 86.0\% & 49.0\% & 62.3\% &- &-&-& 47.5\% \\
MiniGPT-4-7B (I,T)~\cite{zhu2023minigpt} & 36.06\% & 29.31\% & - & 23.0\% & -& - & 42.84\% & 22.1\% & -& - & - \\
LLaMA-Adapter-v2-7B (I,T)~\cite{gao2023llama} &-&-&-&39.5\% & -&-&-&31.4\% &-&-&-\\
Qwen-VL-7B$^\ddagger$ (I,T)~\cite{qwen} & - & 58.6\% & 78.8\% & 68.2\% & - & 63.8\% & 56.3\% & - & -& - & - \\
MobileVLM-3B (I,T)~\cite{chu2023mobilevlm} & - & - & - & 59.6\% & 84.9\% & 47.5\% & - & - & - & - & -\\
LLaVA-Phi-3B (I,T)~\cite{zhu2024llava_phi} & -& -& 71.4\% & 59.8\% & 85.0\% & 48.6\% & -&28.9\% & - & - & - \\
{Single-Modality-Expert-Task2} (I,T) & 67.07\% & 62.91\% & 75.18\% & 71.26\% & 84.7\% & 45.16\%& 60.63\%& 27.8\% &-&-&- \\
{Single-Modality-Expert-Task5} (I,T,S) & 58.86\% & 56.01\% & 67.35\% & 65.80\% &62.48\% &43.78\% &53.50\%  &26.9\% &  30.78\%/24.90\% & 9.33\%/12.00\% & -\\
{Single-Modality-Expert-Task6} (I,T,S) & 58.69\% & 57.77\% & 68.74\% & 67.53\%  &65.84\% &44.24\% &55.21\% &25.6\%  &32.59\%/29.02\% & 18.67\%/8.00\%&-\\
%{Single-Modality-Expert-Task2} & 21.21\% & 32.20\% & 33.26\% & 65.36\%  \\
%{Single-Modality-Expert-Task5} & 14.45\% & 22.68\% & 26.71\% & 62.03\%  \\
%{Single-Modality-Expert-Task6} & 15.69\% & 24.36\% & 26.77\% & 61.05\%  \\
\hline
Sparse Model  & & & & & & & & & \\
MoE-Lla\\

%{Uni-MoE w/ MoE-Task1 1 epoch} & 19.01\% & 30.12\% & 31.05\% & 56.84\%  \\
%{Uni-MoE w/ MoE-Task1 2 epoch} & 19.16\% & 26.84\% & 29.97\% & 56.84\%  \\
%{Uni-MoE w/ MoE-Task1 3 epoch} & 17.48\% & 25.46\% & 28.50\% & 55.43\%  \\ 
%{Uni-MoE w/ MoE-Task1-short 1 epoch} & 22.11\% & 33.12\% & 32.49\% & 54.54\% \\
%{Uni-MoE w/ MoE-Task1-short 2 epoch} & 22.97\% & \textbf{36.18}\% & 33.36\% & 63.06\% \\
%{Uni-MoE w/ MoE-Task1-short 3 epoch} & \textbf{25.14\%} & 34.64\% & 35.17\% & 62.37\% \\

%{Uni-MoE w/ MoE-Task1 1 epoch} & 62.88\% & 57.77\% & 69.82\% & 68.84\%  \\
{Uni-MoE w/ MoE-Task1 (4E)} (I,T,S) & 61.22\% & 57.63\% & 68.42\% & 68.15\% &56.67\% & 39.12\% & 52.58\% &30.1\% & 47.08\%/47.08\% & 41.33\%/36.00\% & - \\
%{Uni-MoE w/ MoE-Task1 3 epoch} & 59.91\% & 57.07\% & 68.05\% & 67.28\%  \\ 
%{Uni-MoE w/ MoE-Task2 1 epoch} & 66.20\% & 63.02\% & 74.41\% & 71.17\%  \\
{Uni-MoE w/ MoE-Task2 (4E)} (I,T,S,V)& 65.07\% & 62.10\% & 73.87\% & 70.50\% & 85.43\% &41.56\% &60.54\% &28.2\% & 49.65\% /49.37\% & 42.00\%/48.00\% & 42.2\% \\
%{Uni-MoE w/ MoE-Task3 1 epoch} & 65.07\% & 61.38\% & 73.66\% & 69.52\%  \\
{Uni-MoE w/ MoE-Task3 (4E)} (I,T,A,V) & 64.28\% & 61.96\% & 73.87\% & 69.82\% & 86.10\% & 40.63\% &59.16\% &31.7\% & - & 42.8\% \\
%{Uni-MoE w/ MoE-Task2 1 epoch} & 22.93\% & 32.98\% & 35.80\% & 60.54\%  \\
%{Uni-MoE w/ MoE-Task2 2 epoch} & 24.14\% & 34.72\% & 37.98\% & 59.79\%  \\
%{Uni-MoE w/ MoE-Task3 1 epoch} & 23.43\% & 35.06\% & \textbf{38.54}\% & 67.12\%  \\
%{Uni-MoE w/ MoE-Task3 2 epoch} & 22.76\% & 35.18\% & 37.51\% & \textbf{67.47}\%  \\
{Uni-MoE w/ MoE-Task4 (4E)} (I,T,S,V) & 69.08\% & 66.02\% & 76.4\% & 73.3\% & 86.0\% & 49.2\% & 63.4\% & 32.6\% & 64.21\%/64.72\% & 48.00\%/58.67\% & 45.6\%\\
+ Aux\_loss & 69.61\% & 66.13\%& 76.0\%& 72.6\%&  84.8\%  & 48.2\% & 63.3\% & 31.7\% & 63.86\%/64.24\%& 50.00\%/54.00\% & 45.2\%\\
{Uni-MoE w/ MoE-Task4 (8E)} (I,T,S,V) \\
+ Aux\_loss \\
\hline
\end{tabular}}

\end{table*}



\begin{table}[t]
\renewcommand\arraystretch{1.15}
\centering
\caption{\label{image-text-und}
\textbf{Model performance on image-text understanding and reasoning benchmarks}. Uni-MoE still achieves better performance compared to models with the single expert configuration.}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|cccc}
\hline
\textbf{Method} & \textbf{A-OKVQA} & \textbf{OK-VQA} & \textbf{VQAv2} & \textbf{MMBench} \\
\hline
Macaw-LLM~\cite{lyu2023macaw}  & 1.90\% & 5.70\% & 20.73\% & 3.84\%  \\
X-InstructBLIP~\cite{panagopoulou2023x} & 21.52\% & 30.61\% & 37.77\% & 8.96\% \\
\hline
{Single-Modality-Expert-Task2} & 67.07\% & 62.91\% & 75.18\% & 71.26\%  \\
{Single-Modality-Expert-Task5} & 58.86\% & 56.01\% & 67.35\% & 65.80\%  \\
{Single-Modality-Expert-Task6} & 58.69\% & 57.77\% & 68.74\% & 67.53\%  \\
%{Single-Modality-Expert-Task2} & 21.21\% & 32.20\% & 33.26\% & 65.36\%  \\
%{Single-Modality-Expert-Task5} & 14.45\% & 22.68\% & 26.71\% & 62.03\%  \\
%{Single-Modality-Expert-Task6} & 15.69\% & 24.36\% & 26.77\% & 61.05\%  \\
\hline
%{Uni-MoE w/ MoE-Task1 1 epoch} & 19.01\% & 30.12\% & 31.05\% & 56.84\%  \\
%{Uni-MoE w/ MoE-Task1 2 epoch} & 19.16\% & 26.84\% & 29.97\% & 56.84\%  \\
%{Uni-MoE w/ MoE-Task1 3 epoch} & 17.48\% & 25.46\% & 28.50\% & 55.43\%  \\ 
%{Uni-MoE w/ MoE-Task1-short 1 epoch} & 22.11\% & 33.12\% & 32.49\% & 54.54\% \\
%{Uni-MoE w/ MoE-Task1-short 2 epoch} & 22.97\% & \textbf{36.18}\% & 33.36\% & 63.06\% \\
%{Uni-MoE w/ MoE-Task1-short 3 epoch} & \textbf{25.14\%} & 34.64\% & 35.17\% & 62.37\% \\

{Uni-MoE w/ MoE-Task1 1 epoch} & 62.88\% & 57.77\% & 69.82\% & 68.84\%  \\
{Uni-MoE w/ MoE-Task1 2 epoch} & 61.22\% & 57.63\% & 68.42\% & 68.15\%  \\
{Uni-MoE w/ MoE-Task1 3 epoch} & 59.91\% & 57.07\% & 68.05\% & 67.28\%  \\ 
{Uni-MoE w/ MoE-Task2 1 epoch} & 66.20\% & 63.02\% & 74.41\% & 71.17\%  \\
{Uni-MoE w/ MoE-Task2 2 epoch} & 65.07\% & 62.10\% & 73.87\% & 70.50\%  \\
{Uni-MoE w/ MoE-Task3 1 epoch} & 65.07\% & 61.38\% & 73.66\% & 69.52\%  \\
{Uni-MoE w/ MoE-Task3 2 epoch} & 64.28\% & 61.96\% & 73.87\% & 69.82\%  \\
%{Uni-MoE w/ MoE-Task2 1 epoch} & 22.93\% & 32.98\% & 35.80\% & 60.54\%  \\
%{Uni-MoE w/ MoE-Task2 2 epoch} & 24.14\% & 34.72\% & 37.98\% & 59.79\%  \\
%{Uni-MoE w/ MoE-Task3 1 epoch} & 23.43\% & 35.06\% & \textbf{38.54}\% & 67.12\%  \\
%{Uni-MoE w/ MoE-Task3 2 epoch} & 22.76\% & 35.18\% & 37.51\% & \textbf{67.47}\%  \\
\hline
\end{tabular}}

\end{table}



\begin{table}[t]
\centering
\renewcommand\arraystretch{1.15}
\caption{\label{hign_school}
 \textbf{Zero-shot Results on our collected English High School Listening Test (Long Speech)}. It aims to assess the long/short speech understanding abilities of MLLMs in real-world applications of speech recognition.}
\resizebox{0.90\linewidth}{!}{
\begin{tabular}{l|cc}
\hline
\textbf{Method} & \textbf{Long} & \textbf{Short}\\
\hline
{Macaw-LLM~\cite{lyu2023macaw}}&0.67\%&2.00\%\\
X-InstructBLIP~\cite{panagopoulou2023x} & 0.67\% & 2.00\% \\
\hline
Single-Modality-Expert-Task4 & 12.67\% & 6.00\% \\
Single-Modality-Expert-Task5 & 9.33\% & 12.00\% \\
{Single-Modality-Expert-Task6} & 18.67\% & 8.00\% \\
{Single-Modality-Expert-Task7} & 34.67\% & 46.00\% \\
\hline
%{Uni-MoE w/ MoE-Task1 1 epoch} & 32.67\% & 38.00\% \\
{Uni-MoE w/ MoE-Task1 2 epoch} & 41.33\% & 36.00\% \\
%{Uni-MoE w/ MoE-Task2 1 epoch} & \textbf{43.33\%} & 36.00\% \\
{Uni-MoE w/ MoE-Task2 2 epoch} & \textbf{42.00\%} & \textbf{48.00\%} \\
\hline
\end{tabular}}

\end{table}

==> all_experimental_results.tex <==
\subsection*{original tables}
\begin{table*}[htbp]
\centering
\small
\begin{tabular}{llllll}
\hline
\textbf{baselines} & \textbf{A-OK-VQA} & \textbf{OK-VQA} & \textbf{VQA2} & \textbf{MMBench (hint:long speech)} & \textbf{RACE (held\_in)}\\
\hline
{llava-150k-instruct-audio} & \verb|18.38%| & \verb|26.58%| & \verb|32.60%| & \verb|-|  & \verb|-| \\
{llava-150k-instruct-text} & \verb|21.21%| & \verb|32.20%| & \verb|33.26%| & \verb|65.36%(45.34%)|  & \verb|-| \\
{llava-150k-instruct-audio*} & \verb|19.26%| & \verb|27.68%| & \verb|32.95%| & \verb|-|  & \verb|-| \\
{longspeech+llava-150k-instruct-audio} & \verb|9.14%| & \verb|12.26%| & \verb|24.30%| & \verb|-|  & \verb|-| \\
{longspeech+llava-150k-instruct} & \verb|4.56%| & \verb|3.42%| & \verb|5.90%| & \verb|-|  & \verb|-| \\
{longspeech+llava-150k-instruct+*-audio} & \verb|11.40%| & \verb|14.40%| & \verb|25.11%| & \verb|61.05%(47.52%)|  & \verb|-| \\
{longspeech with choice} & \verb|-| & \verb|-| & \verb|-| & \verb|57.37%(47.83%)| & \makecell{ middle:46.80\% \\ high:48.74\% } \\
{moe 2 experts} & \verb|12.55%| & \verb|18.42%| & \verb|25.83%| & \verb|56.41%(49.38%)| & \makecell{ middle:40.95\% \\ high:40.39\% } \\
{moe 2 experts} & \verb|13.52%| & \verb|15.92%| & \verb|26.77%| & \verb|53.99%(48.45%)| & \makecell{ middle:42.62\% \\ high:42.40\% } \\
{moe 2 experts new 1epoch} & \makecell{19.02\%\\23.53\%} & \makecell{26.26\%\\32.86\%} & \makecell{33.10\%\\37.24\%} & \makecell{58.94\%\\hint:43.79\%} & \makecell{ middle:41.71\% \\ high:41.37\% } \\
{moe 2 experts new 2epoch} & \makecell{19.23\%\\23.96\%} & \makecell{26.58\%\\32.76\%} & \makecell{31.47\%\\35.02\%} & \makecell{59.97\%\\hint:48.45\%} & \makecell{ middle:- \\ high:- } \\
{moe 2 experts new 3epoch} & \makecell{18.81\%\\23.00\%} & \makecell{27.86\%\\33.42\%} & \makecell{33.98\%\\36.39\%} & \makecell{59.45\%\\hint:47.52\%} & \makecell{ middle:- \\ high:- } \\
{moe 4 experts 1epoch} & \makecell{16.59\%\\22.11\%} & \makecell{23.60\%\\33.12\%} & \makecell{27.71\%\\32.49\%} & \makecell{24.54\%\\hint:43.17\%} & \makecell{ middle:- \\ high:- } \\
{moe 4 experts 2epoch} & \makecell{19.31\%\\22.97\%} & \makecell{26.46\%\\36.18\%} & \makecell{31.28\%\\33.36\%} & \makecell{63.06\%\\hint:37.58\%} & \makecell{ middle:- \\ high:- } \\
{moe 4 experts 3epoch} & \makecell{20.01\%\\25.14\%} & \makecell{29.04\%\\34.64\%} & \makecell{30.86\%\\35.17\%} & \makecell{62.37\%\\hint:34.78\%} & \makecell{ middle:- \\ high:- } \\
{moe 4 experts 1epoch full data} & \makecell{14.79\%\\19.01\%} & \makecell{20.04\%\\30.12\%} & \makecell{28.59\%\\31.05\%} & \makecell{56.84\%\\hint:48.76\%}  & \makecell{ middle:43.38\% \\ high:44.00\% } \\
{moe 4 experts 2epoch full data} & \makecell{14.80\%\\19.16\%} & \makecell{19.98\%\\26.84\%} & \makecell{26.01\%\\29.97\%} & \makecell{56.84\%\\hint:44.41\%}  & \makecell{ middle:47.08\% \\ high:47.08\% } \\
{moe 4 experts 3epoch full data} & \makecell{13.58\%\\17.48\%} & \makecell{17.68\%\\25.46\%} & \makecell{20.14\%\\28.50\%} & \makecell{55.43\%\\hint:47.20\%}  & \makecell{ middle:50.77\% \\ high:48.94\% } \\
{moe 4 3causal1} & \verb|-(-)| & \verb|-(-)| & \verb|-(-)| & \makecell{64.52\%\\hint:44.41\%} & \makecell{ middle:31.34\% \\ high:31.62\% } \\
{moe 4 3causal2} & \verb|-(-)| & \verb|-(-)| & \verb|-(-)| & \makecell{64.88\%\\hint:49.69\%} & \makecell{ middle:33.91\% \\ high:37.22\% } \\
{moe 4 3causal3} & \verb|-(-)| & \verb|-(-)| & \verb|-(-)| & \makecell{65.11\%\\hint:48.14\%} & \makecell{ middle:36.63\% \\ high:37.45\% } \\
{moe 4 3causal4} & \verb|-(-)| & \verb|-(-)| & \verb|-(-)| & \makecell{65.48\%\\hint:44.10\%} & \makecell{ middle:37.74\% \\ high:38.16\% } \\
{moe 4 3causal5} & \verb|-(-)| & \verb|-(-)| & \verb|-(-)| & \makecell{64.31\%\\hint:47.52\%} & \makecell{ middle:34.68\% \\ high:35.68\% } \\
{moe 4 3causal7} & \verb|-(-)| & \verb|-(-)| & \verb|-(-)| & \makecell{64.66\%\\hint:48.45\%} & \makecell{ middle:39.35\% \\ high:39.08\% } \\
{moe 4 vqa epoch1} & \makecell{2.80\%\\9.70\%} & \makecell{5.38\%\\14.18\%} & \makecell{9.85\%\\13.92\%} & \makecell{-\%\\hint:-\%}  & \makecell{ middle:-\% \\ high:-\% } \\
{moe 4 speech video epoch1} & \makecell{7.37\%\\22.93\%} & \makecell{8.50\%\\32.98\%} & \makecell{10.46\%\\35.80\%} & \makecell{60.54\%\\hint:48.76\%}  & \makecell{ middle:46.31\% \\ high:43.71\% } \\
{moe 4 speech video epoch2} & \makecell{7.76\%\\24.14\%} & \makecell{8.08\%\\34.72\%} & \makecell{12.68\%\\37.98\%} & \makecell{59.79\%\\hint:49.38\%}  & \makecell{ middle:49.65\% \\ high:49.37\% } \\

{moe 4 cap video epoch1} & \makecell{23.43\%} & \makecell{35.06\%} & \makecell{38.54\%} & \makecell{67.12\%}  & \makecell{-} \\
{moe 4 cap video epoch2} & \makecell{22.76\%} & \makecell{35.18\%} & \makecell{37.51\%} & \makecell{67.47\%}  & \makecell{-} \\
{moe 4 cappre video epoch1} & \makecell{20.18\%} & \makecell{32.90\%} & \makecell{36.91\%} & \makecell{60.91\%}  & \makecell{-} \\
{moe 6 cap video epoch1} & \makecell{22.34\%} & \makecell{32.26\%} & \makecell{37.31\%} & \makecell{48.41\%}  & \makecell{-} \\
{macaw} & \makecell{1.08\%\\1.90\%} & \makecell{1.06\%\\5.70\%} & \makecell{2.33\%\\20.73\%} & \makecell{3.84\%\\hint:1.86\%}  & \makecell{ middle:4.04\% \\ high:3.00\% } \\
{xinstruct} & \makecell{0.91\%\\22.52\%} & \makecell{0.00\%\\30.61\%} & \makecell{26.47\%\\34.43\%} & \makecell{8.96\%\\hint:11.23\%}  & \makecell{ middle:16.33\% \\ high:18.88\% } \\
\hline
\end{tabular}
\caption{\label{citation-guide}
baselines for llava-based model via whisper encoder. MMBench: hint for held-out testing of long speech and original testing of image-text reasoning.}
\end{table*}

\begin{table*}[htbp]
\centering
\begin{tabular}{lll}
\hline
\textbf{baselines} & \textbf{long} & \textbf{short}\\
\hline
{longspeech with choice} & \verb|34.67%| & \verb|46.00%| \\
{moe 4 experts 1epoch full data} & \verb|32.67%| & \verb|38.00%| \\
{moe 4 experts 2epoch full data} & \verb|41.33%| & \verb|36.00%| \\
{moe 4 speech video epoch1} & \verb|43.33%| & \verb|36.00%| \\
{moe 4 speech video epoch2} & \verb|38.00%| & \verb|48.00%| \\
\hline
\end{tabular}
\caption{\label{citation-guide}
baselines for English high school exam listerning part.}
\end{table*}

\begin{table*}[htbp]
\centering
\begin{tabular}{llll}
\hline
\textbf{baselines} & \textbf{ClothoAQA} & \textbf{ClothoV1} & \textbf{ClothoV2}\\
\hline
{beats ft epoch1} & \verb|31.61%| & \verb|19.1%| & \verb|18.7%| \\
{beats ft epoch2} & \verb|32.31%| & \verb|22.3%| & \verb|21.6%| \\
{beats ft epoch3} & \verb|31.39%| & \verb|20.2%| & \verb|19.2%| \\
{moe 4 cap video epoch1} & \verb|32.59%| & \verb|25.0%| & \verb|24.7%| \\
{moe 4 cap video epoch2} & \verb|31.07%| & \verb|24.8%| & \verb|25.1%| \\
{moe 4 cappre video epoch1} & \verb|20.31%| & \verb|21.0%| & \verb|21.2%| \\
{moe 6 cappre video epoch1} & \verb|27.74%| & \verb|20.3%| & \verb|21.8%| \\
{xinstruct} & \verb|15.4%| & \verb|29.4%| & \verb|27.4%| \\
\hline
\end{tabular}
\caption{\label{citation-guide}
baselines for audio captioning.}
\end{table*}


\begin{table*}[htbp]
\centering
\begin{tabular}{lll}
\hline
\textbf{baselines} & \textbf{ActivityNet} & \textbf{MSVD} \\
\hline
{Gemini} & \verb|52.2| & \verb|-| \\
{FrozenBiLM} & \verb|24.7| & \verb|32.2| \\
{VideoChat} & \verb|26.5/2.2| & \verb|56.3/2.8| \\
{LLaMA-Adapter} & \verb|34.5/2.7| & \verb|54.9/3.1| \\
{Video-LLaMA} & \verb|12.4/1.1| & \verb|51.6/2.5| \\
{Video-ChatGPT} & \verb|35.2/2.7| & \verb|64.9/3.3| \\
{Chat-UniVi} & \verb|45.8/3.2| & \verb|65.0/3.6| \\
{Video-LLaVA} & \verb|45.3/3.3| & \verb|70.7/3.9| \\
{PG-Video-LLaVA} & \verb|39.9/3.3| & \verb|64.1/3.7| \\
{LLaMA-VID Vicuna-7B} & \verb|47.4/3.3| & \verb|69.7/3.7| \\
{LLaMA-VID Vicuna-13B} & \verb|47.5/3.3| & \verb|70.0/3.7| \\
\hline
{Ours speech epoch1} & \verb|42.7/2.5| & \verb|55.0/3.2| \\
{Ours speech epoch2} & \verb|42.2/2.5| & \verb|55.3/3.2| \\
{Ours speech epoch3} & \verb|41.9/2.5| & \verb|54.3/3.1| \\
{Ours cap epoch1} & \verb|42.7/2.5| & \verb|55.6/3.4| \\
{Ours cap epoch2} & \verb|42.1/2.8| & \verb|56.1/3.4| \\
{Ours cappre epoch1} & \verb|42.3/2.8| & \verb|58.1/3.5| \\
{Ours 6 cappre epoch1} & \verb|43.8/2.6| & \verb|58.3/3.3| \\
\hline
\end{tabular}
\caption{\label{citation-guide}
baselines for video understanding.}
\end{table*}
